All once-extended 3D TQFTs are Reshetikhin--Turaev theories

We present a direct geometric construction which extends the Reshetikhin--Turaev TQFT to circles. We prove that this agrees with the generators-and-relations approach of Bartlett--Douglas--Schommer-Pries--Vicary, thus providing an alternative to the Cerf-theoretic part of their classification of once-extended 3-dimensional TQFTs, and deduce as a result that all once-extended 3-dimensional TQFTs arise via our construction.

==> arrows.tex <==
\newcommand*\arrowoffset{0.4pt}
\makeatletter
\pgfarrowsdeclare{new double arrowhead}{new double arrowhead}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \advance\pgfutil@tempdimb by \arrowoffset % Jamie addition
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetstrokecolor{black}
  \pgfsetlinewidth{0.6pt}
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-3\pgfutil@tempdima+\arrowoffset}{4\pgfutil@tempdima}}
  \pgfpathcurveto
                {\pgfpoint{-2.75\pgfutil@tempdima+\arrowoffset}{2.5\pgfutil@tempdima}}
                {\pgfpoint{\arrowoffset}{0.25\pgfutil@tempdima}}
                {\pgfpoint{0.75\pgfutil@tempdima+\arrowoffset}{0pt}}
  \pgfpathcurveto
                {\pgfpoint{\arrowoffset}{-0.25\pgfutil@tempdima}}
                {\pgfpoint{-2.75\pgfutil@tempdima+\arrowoffset}{-2.5\pgfutil@tempdima}}
                {\pgfpoint{-3\pgfutil@tempdima+\arrowoffset}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}
\pgfarrowsdeclare{new single arrowhead}{new single arrowhead}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \advance\pgfutil@tempdimb by \arrowoffset % Jamie addition
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetstrokecolor{black}
  \pgfsetlinewidth{0.6pt}
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
                {\pgfpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
                {\pgfpoint{0pt}{0.25\pgfutil@tempdima}}
                {\pgfpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
                {\pgfpoint{0pt}{-0.25\pgfutil@tempdima}}
                {\pgfpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
                {\pgfpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}
\makeatother
\def\proarrow{\relbar\joinrel\mapstochar\joinrel\rightarrow}
% Produces an autogrowing mapsto arrow
\makeatletter
\tikzset{nomorepostaction/.code={\let\tikz@postactions\pgfutil@empty}}
\makeatother
\tikzset{double arrow scope/.style={\ignore{every node/.style={font=\scriptsize},}every path/.style={
        double, -new double arrowhead}}}
\newcommand\doubleto[1][0.5]{\mathbin{\ensuremath{\begin{tikzpicture}
   \node (A) at (0,0) [inner xsep=1.2pt] {};
   \node (B) at (#1,0) [inner xsep=1pt] {};
   \draw [double, -new double arrowhead] (A) to (B);
\end{tikzpicture}}}}
\renewcommand\to[0]{\mathbin{\ensuremath{\begin{tikzpicture}
   \node (A) at (0,0) [inner xsep=1.2pt] {};
   \node (B) at (0.5,0) [inner xsep=1pt] {};
   \draw [-new single arrowhead] (A) to (B);
\end{tikzpicture}}}}
\newcommand\xdoubleto[1]{\mathbin{\begin{tikzpicture}[baseline={([yshift=-2pt]
current bounding box.south)}]\node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=0.2cm, font=\scriptsize] {\ensuremath{\smash{#1\strut}}};\draw [double,-new double arrowhead] ([xshift=-2.5pt] A.south west) to ([xshift=3pt] A.south east);\end{tikzpicture}}}

\newcommand\longxdoubleto[2][0.5cm]{\mathbin{\begin{tikzpicture}[baseline={([yshift=1pt]current bounding box.south)}]\node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=#1] {\ensuremath{#2}};\path [use as bounding box] ([xshift=-2.5pt, yshift=-3pt] A.south west) rectangle ([xshift=2.5pt] A.north east);\draw [double,-new double arrowhead] ([xshift=-2.5pt] A.south west) to ([xshift=3pt] A.south east);
\end{tikzpicture}}}

\newcommand\xleftdoubleto[1]{\mathbin{\begin{tikzpicture}[baseline={([yshift=-3pt]
current bounding box.south)}]
    \node (A) at (0,0) [inner xsep=0pt, inner ysep=-1pt, minimum width=0.2cm] {\ensuremath{\scriptstyle #1 \strut}};
    \draw [double,new double arrowhead-]
        ([xshift=-2.5pt] A.south west)
        to ([xshift=3pt] A.south east);
\end{tikzpicture}}}
\newcommand\xto[1]{\mathbin{\begin{tikzpicture}[baseline={([yshift=-3pt]
current bounding box.south)}]
    \node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=0.2cm] {$\scriptstyle #1$};
    \draw [-new single arrowhead]
        ([xshift=-2.5pt] A.south west)
        to ([xshift=3pt] A.south east);
\end{tikzpicture}}}
\newcommand\xyto[2]{\mathbin{\begin{tikzpicture}[baseline={([yshift=10pt]
current bounding box.south)}]
    \node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=0.2cm] {$\scriptstyle #1$};
    \draw [-new single arrowhead]
        ([xshift=-2.5pt] A.south west)
        to node [below] {\ensuremath{#2}} ([xshift=3pt] A.south east);
\end{tikzpicture}}}
\newcommand\longxyto[3]{\mathbin{\begin{tikzpicture}[baseline={([yshift=10pt]
current bounding box.south)}]
    \node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=#3] {$\scriptstyle #1$};
    \draw [-new single arrowhead]
        ([xshift=-0.75pt] A.south west)
        to node [below] {\ensuremath{#2}} ([xshift=-0.25pt] A.south east);
\end{tikzpicture}}}
\newcommand\xmapsto[1]{\mathbin{\begin{tikzpicture}[baseline={([yshift=-3pt]
current bounding box.south)}]
    \node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=0.2cm] {$#1$};
    \draw [|-new single arrowhead]
        ([xshift=-2.5pt] A.south west)
        to ([xshift=3pt] A.south east);
\end{tikzpicture}}}
\newcommand\xleftto[1]{\ignore{\tikzexternalenable}\mathbin{\begin{tikzpicture}[baseline={([yshift=-3pt]
current bounding box.south)}]
    \node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=0.2cm] {$\scriptstyle #1$};
    \draw [new single arrowhead-]
        ([xshift=-2.5pt] A.south west)
        to ([xshift=3pt] A.south east);
\end{tikzpicture}}\ignore{\tikzexternaldisable}}
\newcommand\xleftmapsto[1]{\mathbin{\begin{tikzpicture}[baseline={([yshift=-3pt]
current bounding box.south)}]
    \node (A) at (0,0) [inner xsep=0pt, inner ysep=2pt, minimum width=0.2cm] {$\scriptstyle #1$};
    \draw [new single arrowhead-|]
        ([xshift=-2.5pt] A.south west)
        to ([xshift=3pt] A.south east);
\end{tikzpicture}}}
\newcommand\longxarrow[2]{\mathbin{\begin{tikzpicture}[baseline={([yshift=-2pt]
current bounding box.south)}]
   \node (1) at (0,0) [inner sep=1pt] {};
   \node (2) at (#2,0) [inner sep=1pt] {};
   \draw [-new single arrowhead] (1) to node [above, inner xsep=0pt, inner ysep=2pt]
{\ensuremath{\scriptstyle #1}} (2);
\end{tikzpicture}}}
\newcommand\longxmapsto[2]{\mathbin{\begin{tikzpicture}[baseline={([yshift=-2pt]
current bounding box.south)}]
   \node (1) at (0,0) [inner sep=1pt] {};
   \node (2) at (#2,0) [inner sep=1pt] {};
   \draw [|-new single arrowhead] (1) to node [above, inner xsep=0pt, inner ysep=2pt]
{\ensuremath{\scriptstyle #1}} (2);
\end{tikzpicture}}}
\renewcommand\xrightarrow[1]{\xto{#1}}
\renewcommand\xleftarrow[1]{\xleftto{#1}}
\newcommand\doublearrowspace{15pt}
\newcommand\rightleftdoublearrow[2]{\mathbin{\begin{array}{@{}c@{}}#1\\[-6pt]\,\xdoubleto{\hspace{\doublearrowspace}}\\[-10pt]\xleftdoubleto{\hspace{\doublearrowspace}}\,\\[-6pt]#2\end{array}}}
\newcommand\leftrightdoublearrow[2]{\mathbin{\begin{array}{@{}c@{}}#1\\[-11pt]\xleftdoubleto{\hspace{\doublearrowspace}}\,\\[-10pt]\,\xdoubleto{\hspace{\doublearrowspace}}\\[-6pt]#2\end{array}}}
\newcommand\rightleftmapstodoublearrow[2]{\begin{array}{@{}c@{}}#1\\[-6pt]\xmapsto{\hspace{\doublearrowspace}}\\[0pt]\xleftmapsto{\hspace{\doublearrowspace}}\\[-6pt]#2\end{array}}
